Mode visualisation and control of complex lasers using neural networks

Understanding the behaviour of complex laser systems is an outstanding challenge, especially in the presence of nonlinear interactions between modes. Hidden features, such as the gain distributions and spatial localisation of lasing modes, often cannot be revealed experimentally, yet they are crucial to determining the laser action. Here, we introduce a lasing spectroscopy method that can visualise the gain profiles of the modes in complex lasers using an artificial neural network. The spatial gain distributions of different lasing modes in a disorderly coupled microring array are reconstructed without prior knowledge of the laser topology. We further extend the neural network to a tandem neural network that can control the laser emission by matching the modal gain/loss profile to selectively enhance the targeted modes. This mode visualisation method offers a new approach to extracting hidden spatial mode features from photonic structures, which could improve our understanding and control of complex photonic systems.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
